RMS: Redundancy-Minimizing Point Cloud Sampling for Real-Time Pose Estimation

The typical point cloud sampling methods used in state estimation for mobile robots preserve a high level of point redundancy. This redundancy unnecessarily slows down the estimation pipeline and may cause drift under real-time constraints. Such undue latency becomes a bottleneck for resource-constrained robots (especially UAVs), requiring minimal delay for agile and accurate operation. We propose a novel, deterministic, uninformed, and single-parameter point cloud sampling method named RMS that minimizes redundancy within a 3D point cloud. In contrast to the state of the art, RMS balances the translation-space observability by leveraging the fact that linear and planar surfaces inherently exhibit high redundancy propagated into iterative estimation pipelines. We define the concept of gradient flow, quantifying the local surface underlying a point. We also show that maximizing the entropy of the gradient flow minimizes point redundancy for robot ego-motion estimation. We integrate RMS into the point-based KISS-ICP and feature-based LOAM odometry pipelines and evaluate experimentally on KITTI, Hilti-Oxford, and custom datasets from multirotor UAVs. The experiments demonstrate that RMS outperforms state-of-the-art methods in speed, compression, and accuracy in well-conditioned as well as in geometrically-degenerated settings.

==> fig/convergence_analysis/eigenvalues.tex <==
\begin{tikzpicture}[
    >=latex,
    font=\scriptsize
  ]

  \pgfplotstableread[col sep=space]{./data/convergence_analysis/011_sim_x_icp_1/00000_VANILLA.csv}{\tableVANILLA}
  \pgfplotstableread[col sep=space]{./data/convergence_analysis/011_sim_x_icp_1/00013.csv}{\tableRISD}
  \pgfplotstableread[col sep=space]{./data/convergence_analysis/011_sim_x_icp_1/NORMAL_SAMPLING.csv}{\tableNS}
  
  \begin{axis}[ 
    name=ex,
    width=0.52\columnwidth,
    height=0.25\columnwidth,
    grid=major,
    grid style={draw=gray!30,line width=.1pt},
    ylabel=$\lambda_1$,
    ylabel shift=-3pt,
    xticklabels={},
    ytick={0, 100},
    enlarge x limits=0,
    axis line style={latex-latex},
    yshift=0.6em,
    legend columns=3,
    legend style={text=black, fill=none, draw=none, at={(1.03, 1.6)}, line width=2pt},
    ]
    \addplot [smooth, color=color_blue, line width=0.5pt] table [y=e_x, x=ts]{\tableVANILLA};
    \addplot [smooth, color=color_green, line width=0.5pt] table [y=e_x, x=ts]{\tableNS};
    \addplot [smooth, color=color_red, line width=0.5pt] table [y=e_x, x=ts]{\tableRISD};

    \addlegendentry{\tiny{V40}}
    \addlegendentry{\tiny{V20+NS}}
    \addlegendentry{\tiny{V20+RISE}}
  \end{axis}

  \begin{axis}[ 
    name=ey,
    at=(ex.below south west), anchor=above north west,
    width=0.52\columnwidth,
    height=0.25\columnwidth,
    grid=major,
    grid style={draw=gray!30,line width=.1pt},
    ylabel=$\lambda_2$,
    ylabel shift=-3pt,
    xticklabels={},
    ytick={0, 100},
    enlarge x limits=0,
    axis line style={latex-latex},
    yshift=0.6em,
    ]
    \addplot [smooth, color=color_blue, line width=0.5pt] table [y=e_y, x=ts]{\tableVANILLA};
    \addplot [smooth, color=color_green, line width=0.5pt] table [y=e_y, x=ts]{\tableNS};
    \addplot [smooth, color=color_red, line width=0.5pt] table [y=e_y, x=ts]{\tableRISD};
  \end{axis}

  \begin{axis}[ 
    name=ez,
    at=(ey.below south west), anchor=above north west,
    width=0.52\columnwidth,
    height=0.25\columnwidth,
    grid=major,
    grid style={draw=gray!30,line width=.1pt},
    xlabel=time (s),
    xlabel shift=-5pt,
    ylabel=$\lambda_3$,
    ylabel shift=-3pt,
    ytick={0, 150},
    % xtick={0, 50, 100},
    enlarge x limits=0,
    enlarge y limits=0.2,
    axis line style={latex-latex},
    yshift=0.6em,
    ]
    \addplot [smooth, color=color_blue, line width=0.5pt] table [y=e_z, x=ts]{\tableVANILLA};
    \addplot [smooth, color=color_green, line width=0.5pt] table [y=e_z, x=ts]{\tableNS};
    \addplot [smooth, color=color_red, line width=0.5pt] table [y=e_z, x=ts]{\tableRISD};
  \end{axis}

\end{tikzpicture}
\vspace{-0.2cm}


==> fig/motivation.tex <==
% \pgfdeclarelayer{background}
% \pgfdeclarelayer{foreground}
% \pgfsetlayers{background,main,foreground}
\usetikzlibrary{
  matrix,
}

% legend line style
\pgfplotsset{
  compat=1.6,
  legend image code/.code={
    \draw[mark repeat=2,mark phase=2]
    plot coordinates {
      (0cm,0cm)
      (0.15cm,0cm)        %% default is (0.3cm,0cm)
      (0.3cm,0cm)         %% default is (0.6cm,0cm)
    };%
  }
}

\begin{tikzpicture}[|every node/.style={
  inner sep = .01em,
  outer sep=0.02em,
  text centeblue,
  minimum height = .5em},
  >=latex,
  font=\scriptsize
  ]

  \tikzstyle{legend_style} = [fill=black, line width=0.3mm]

  \node[anchor=south west,inner sep=0] (a) at (0,0) {
      \def\arraystretch{0}%
      \includegraphics[width=0.95\columnwidth]{\FIGPATH/motivation_robots.jpg}%
    }; 
  \begin{scope}[x={(a.south east)},y={(a.north west)}]

    % %%{ useful grid to help you find coordinates for plotting the overlay
    % \draw[black, xstep=.1, ystep=.1] (0,0) grid (1,1);
    % \foreach \i in {0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1} {
    %   \node[align=center] at (\i, -0.05) {\i};
    %   \node[align=center] at (\i, 1.05) {\i};
    %   \node[align=center] at (-0.05, \i) {\i};
    %   \node[align=center] at (1.05, \i) {\i};
    % }
    % %%}

    % draw axes labels
    % \node [] at (0.8, 0.00) {x (m)};
    % \node [rotate=90] at (0.54, 0.5) {y (m)};

    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.026, 0.963) {\scriptsize \textbf{a)}};
    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.533, 0.963) {\scriptsize \textbf{b)}};
    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.026, 0.490) {\scriptsize \textbf{c)}};
    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.483, 0.490) {\scriptsize \textbf{d)}};
    % \node[] at (0.52, 0.95) {\scriptsize \textbf{b)}};

  \end{scope}

  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/GT.tum}{\tableTRAJGT}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/NORMAL_SAMPLING.txt}{\tableTRAJNS}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/UNIFORM_SAMPLING.txt}{\tableTRAJV}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/COVARIANCE_SAMPLING.txt}{\tableTRAJCOV}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/RISE.txt}{\tableTRAJRISE}
  
  \begin{axis}[ 
    name=kitti,
    width=0.53\columnwidth,
    height=0.53\columnwidth,
    xlabel=x (m),
    ylabel=y (m),
    xlabel shift=-1.5mm,
    ylabel shift=-5mm,
    enlarge x limits=0.02,
    enlarge y limits=0.02,
    xshift=5mm,
    axis line style={latex-latex},
    grid=major,
    grid style={draw=gray!10,line width=.05pt},
    ]

  \addplot [smooth, color=black, line width=0.7pt] table [y=y, x=x]{\tableTRAJGT};
  \addplot [smooth, color=color_blue, line width=0.7pt] table [y=y, x=x]{\tableTRAJV};
  \addplot [smooth, color=color_green, line width=0.7pt] table [y=y, x=x]{\tableTRAJNS};
  \addplot [smooth, color=color_orange, line width=0.7pt] table [y=y, x=x]{\tableTRAJCOV};
  \addplot [smooth, color=color_red, line width=0.7pt] table [y=y, x=x]{\tableTRAJRISE};

  \end{axis}

  \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/GT.tum}{\tableTRAJGT}
  \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/NS.tum}{\tableTRAJNS}
  \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/UNIFORM_SAMPLING.tum}{\tableTRAJV}
  \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/COVARIANCE_SAMPLING.tum}{\tableTRAJCOV}
  \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/RISE.tum}{\tableTRAJRISE}
  % \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/map.asc}{\tableMAP}

  % \begin{axis}[ 
  %   name=dronument,
  %   at=(kitti.south east), anchor=south west,
  %   width=0.53\columnwidth,
  %   height=0.53\columnwidth,
  %   xshift=17mm,
  %   yshift=0mm,
  %   grid=major,
  %   grid style={draw=gray!10,line width=.05pt},
  %   xlabel=x (m),
  %   ylabel=y (m),
  %   zlabel=z (m),
  %   ztick={0, 4},
  %   x label style={at={(0.05,0.02)}, rotate=-34},
  %   y label style={at={(0.6,0.00)}, rotate=3},
  %   z label style={at={(-0.08,0.5)}},
  %   enlarge x limits=0,
  %   enlarge y limits=0,
  %   enlarge z limits=0,
  %   view={70}{10},
  %   ]

  %   % \addplot3 [scatter, only marks] table [y=y, x=x, z=z]{\tableMAP};
  %   \addplot3 [smooth, color=black, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJGT}; \label{ground_truth}
  %   \addplot3 [smooth, color=color_blue, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJV}; \label{uniform_sampling}
  %   \addplot3 [smooth, color=color_green, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJNS}; \label{normal_sampling}
  %   \addplot3 [smooth, color=color_red, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJRISE}; \label{RISE_(proposed)}
            
  %   \coordinate (legend) at (axis description cs:0.08,0.58);

  % \end{axis}

  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-2mm, column sep=-1mm,
  % ] at (legend) {
  %   \ref{ground_truth}     & \hspace{-9mm} ground truth \\
  %   \hspace{0mm} sampling: & \\
  %   \ref{uniform_sampling} & \hspace{-9mm} uniform \\
  %   \ref{normal_sampling}  & \hspace{-9mm} normal \\
  %   \ref{RISE_(proposed)}  & \hspace{-9mm} proposed \\
  % };

  \begin{axis}[ 
    name=dronument,
    at=(kitti.south east), anchor=south west,
    width=0.53\columnwidth,
    height=0.53\columnwidth,
    xshift=8mm,
    yshift=0mm,
    grid=major,
    grid style={draw=gray!10,line width=.05pt},
    xlabel=x (m),
    ylabel=y (m),
    zlabel=z (m),
    ztick={0, 4},
    x label style={at={(-0.05,0.06)}, rotate=-45},
    y label style={at={(0.55,0.00)}, rotate=1},
    z label style={at={(-0.08,0.5)}},
    enlarge x limits=0,
    enlarge y limits=0,
    enlarge z limits=0,
    view={80}{10},
    ]

    % \addplot3 [scatter, only marks] table [y=y, x=x, z=z]{\tableMAP};
    \addplot3 [smooth, color=black, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJGT}; \label{ground_truth}
    \addplot3 [smooth, color=color_blue, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJV}; \label{uniform_sampling}
    \addplot3 [smooth, color=color_green, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJNS}; \label{normal_sampling}
    \addplot3 [smooth, color=color_orange, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJCOV}; \label{covariance_sampling}
    \addplot3 [smooth, color=color_red, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJRISE}; \label{RISE_(proposed)}
            
    \coordinate (gt) at (axis description cs:1.45,0.75);
    \coordinate (legend) at (axis description cs:1.32,-0.12);

  \end{axis}

  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-2mm, column sep=-1mm,
  %   nodes={rotate=0},
  %   font=\scriptsize,
  % ] at (gt) {
  %   \hspace{0mm} \ref{ground_truth} & ground truth  \\
  % };

  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-2mm, column sep=-0mm,
  %   nodes={rotate=0},
  %   font=\scriptsize,
  % ] at (gt) {
  %   \hspace{0mm} \textbf{ground}\\
  %   \hspace{1mm} \textbf{truth}\\
  % };

  \node[fill=none] at (7.8, 3.0) {sampling:};
  % \node[fill=none,rotate=90] at (7.8, 2.3) {\textcolor{color_green}{\textbf{normal}}};
  % \node[fill=none,rotate=90] at (8.1, 2.3) {\textcolor{color_blue}{\textbf{uniform}}};
  % \node[fill=none,rotate=90] at (7.8, 1.0) {\textcolor{color_violet}{\textbf{covariance}}};
  % \node[fill=none,rotate=90] at (8.1, 1.0) {\textcolor{color_red}{\textbf{proposed}}};

  \node[fill=none,rotate=90] at (7.8, 1.7) {\textcolor{color_green}{\textbf{Rusinkiewicz et al.}}};
  \node[fill=none,rotate=90] at (8.1, 2.1) {\textcolor{color_blue}{\textbf{Voxelization}}};
  \node[fill=none,rotate=90] at (7.8, 0.06) {\textcolor{color_red}{\textbf{RMS}}};
  \node[fill=none,rotate=90] at (8.1, 0.5) {\textcolor{color_orange}{\textbf{Gelfand et al.}}};

  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-3mm, column sep=-1mm,
  %   nodes={rotate=0},
  %   font=\scriptsize,
  % ] at (legend) {
  %   % \hspace{0mm} sampling: \\
  %     \hspace{10mm} \rotatebox{90}{\hspace{3mm} \textcolor{color_violet}{\textbf{covariance}}}
  %   & \hspace{0mm} \rotatebox{90}{\hspace{4mm} \textcolor{color_red}{\textbf{proposed}}}\\
  %     \hspace{10mm} \rotatebox{90}{\hspace{0mm} \textcolor{color_green}{\textbf{normal}}}      
  %   & \hspace{0mm} \rotatebox{90}{\hspace{0mm} \textcolor{color_blue}{\textbf{uniform}}}\\
  % };

  % % ORIGINAL
  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-3mm, column sep=-1mm,
  %   nodes={rotate=90},
  %   font=\scriptsize,
  % ] at (legend) {
  %                          % &                            & \hspace{-0mm} uniform\\
  %                          % &                            & \hspace{0mm} \ref{uniform_sampling} \\
  %                          % &                            & \hspace{-3mm} normal\\
  %                          % &                            & \hspace{-11mm} \ref{normal_sampling} \\
  %   % \hspace{-5mm} ground truth & \hspace{0mm} sampling: & \hspace{-2mm} proposed           \\
  %   % \ref{ground_truth}   & & \hspace{0mm}             \hspace{0mm} \ref{RISE_(proposed)}          \\
  %   % \hspace{0mm} \textbf{ground truth} & \\
  %   \hspace{0mm}           & \hspace{1.0mm} \textcolor{color_red}{\textbf{proposed}} \\
  %   \hspace{1mm} sampling: & \hspace{2mm} \textcolor{color_green}{\textbf{normal}} \\
  %   \hspace{0mm}           & \hspace{0mm} \textcolor{color_blue}{\textbf{uniform}} \\
  % };


\end{tikzpicture}
% \vspace{-0.2cm}


==> fig/motivation_2.tex <==
% \pgfdeclarelayer{background}
% \pgfdeclarelayer{foreground}
% \pgfsetlayers{background,main,foreground}
\usetikzlibrary{
  matrix,
}

% legend line style
\pgfplotsset{
  compat=1.6,
  legend image code/.code={
    \draw[mark repeat=2,mark phase=2]
    plot coordinates {
      (0cm,0cm)
      (0.15cm,0cm)        %% default is (0.3cm,0cm)
      (0.3cm,0cm)         %% default is (0.6cm,0cm)
    };%
  }
}

\begin{tikzpicture}[|every node/.style={
  inner sep = .01em,
  outer sep=0.02em,
  text centeblue,
  minimum height = .5em},
  >=latex,
  font=\scriptsize
  ]

  \tikzstyle{legend_style} = [fill=black, line width=0.3mm]

  \node[anchor=south west,inner sep=0] (a) at (0,0) {
      \def\arraystretch{0}%
      \includegraphics[width=0.95\columnwidth]{\FIGPATH/motivation_robots.jpg}%
    }; 
  \begin{scope}[x={(a.south east)},y={(a.north west)}]

    % %%{ useful grid to help you find coordinates for plotting the overlay
    % \draw[black, xstep=.1, ystep=.1] (0,0) grid (1,1);
    % \foreach \i in {0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1} {
    %   \node[align=center] at (\i, -0.05) {\i};
    %   \node[align=center] at (\i, 1.05) {\i};
    %   \node[align=center] at (-0.05, \i) {\i};
    %   \node[align=center] at (1.05, \i) {\i};
    % }
    % %%}

    % draw axes labels
    % \node [] at (0.8, 0.00) {x (m)};
    % \node [rotate=90] at (0.54, 0.5) {y (m)};

    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.026, 0.963) {\scriptsize \textbf{a)}};
    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.533, 0.963) {\scriptsize \textbf{b)}};
    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.026, 0.490) {\scriptsize \textbf{c)}};
    \node[fill=white, draw=white, draw opacity=0.0, fill opacity=0.5, text opacity=1.0] at (0.483, 0.490) {\scriptsize \textbf{d)}};
    % \node[] at (0.52, 0.95) {\scriptsize \textbf{b)}};

  \end{scope}

  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/GT.tum}{\tableTRAJGT}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/NORMAL_SAMPLING.txt}{\tableTRAJNS}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/UNIFORM_SAMPLING.txt}{\tableTRAJV}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/COVARIANCE_SAMPLING.txt}{\tableTRAJCOV}
  \pgfplotstableread[col sep=space]{./fig/motivation/kitti_00/RISE.txt}{\tableTRAJRISE}
  
  \begin{axis}[ 
    name=kitti,
    width=0.53\columnwidth,
    height=0.53\columnwidth,
    xlabel=x (m),
    ylabel=y (m),
    xlabel shift=-1.5mm,
    ylabel shift=-5mm,
    enlarge x limits=0.02,
    enlarge y limits=0.02,
    xshift=5mm,
    axis line style={latex-latex},
    grid=major,
    grid style={draw=gray!10,line width=.05pt},
    ]

  \addplot [smooth, color=black, line width=0.7pt] table [y=y, x=x]{\tableTRAJGT};
  \addplot [smooth, color=color_blue, line width=0.7pt] table [y=y, x=x]{\tableTRAJV};
  \addplot [smooth, color=color_green, line width=0.7pt] table [y=y, x=x]{\tableTRAJNS};
  \addplot [smooth, color=color_orange, line width=0.7pt] table [y=y, x=x]{\tableTRAJCOV};
  \addplot [smooth, color=color_red, line width=0.7pt] table [y=y, x=x]{\tableTRAJRISE};

  \end{axis}

  % \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/GT.tum}{\tableTRAJGT}
  % \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/NS.tum}{\tableTRAJNS}
  % \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/UNIFORM_SAMPLING.tum}{\tableTRAJV}
  % \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/COVARIANCE_SAMPLING.tum}{\tableTRAJCOV}
  % \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/RISE.tum}{\tableTRAJRISE}
  % \pgfplotstableread[col sep=space]{./fig/motivation/stara_voda/map.asc}{\tableMAP}

  % \begin{axis}[ 
  %   name=dronument,
  %   at=(kitti.south east), anchor=south west,
  %   width=0.53\columnwidth,
  %   height=0.53\columnwidth,
  %   xshift=17mm,
  %   yshift=0mm,
  %   grid=major,
  %   grid style={draw=gray!10,line width=.05pt},
  %   xlabel=x (m),
  %   ylabel=y (m),
  %   zlabel=z (m),
  %   ztick={0, 4},
  %   x label style={at={(0.05,0.02)}, rotate=-34},
  %   y label style={at={(0.6,0.00)}, rotate=3},
  %   z label style={at={(-0.08,0.5)}},
  %   enlarge x limits=0,
  %   enlarge y limits=0,
  %   enlarge z limits=0,
  %   view={70}{10},
  %   ]

  %   % \addplot3 [scatter, only marks] table [y=y, x=x, z=z]{\tableMAP};
  %   \addplot3 [smooth, color=black, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJGT}; \label{ground_truth}
  %   \addplot3 [smooth, color=color_blue, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJV}; \label{uniform_sampling}
  %   \addplot3 [smooth, color=color_green, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJNS}; \label{normal_sampling}
  %   \addplot3 [smooth, color=color_red, line width=0.7pt] table [y=y, x=x, z=z]{\tableTRAJRISE}; \label{RISE_(proposed)}
            
  %   \coordinate (legend) at (axis description cs:0.08,0.58);

  % \end{axis}

  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-2mm, column sep=-1mm,
  % ] at (legend) {
  %   \ref{ground_truth}     & \hspace{-9mm} ground truth \\
  %   \hspace{0mm} sampling: & \\
  %   \ref{uniform_sampling} & \hspace{-9mm} uniform \\
  %   \ref{normal_sampling}  & \hspace{-9mm} normal \\
  %   \ref{RISE_(proposed)}  & \hspace{-9mm} proposed \\
  % };

  \node[anchor=south west,inner sep=0] (a) at (kitti.south east) {
      \def\arraystretch{0}%
      \includegraphics[width=0.45\columnwidth]{./fig/motivation/stara_voda/stara_voda.png}%
    }; 

  % \begin{axis}[ 
  %   name=dronument,
  %   at=(kitti.south east), anchor=south west,
  %   width=0.53\columnwidth,
  %   height=0.53\columnwidth,
  %   xshift=8mm,
  %   yshift=0mm,
  %   grid=major,
  %   grid style={draw=gray!10,line width=.05pt},
  %   xlabel=x (m),
  %   ylabel=y (m),
  %   zlabel=z (m),
  %   ztick={0, 4},
  %   x label style={at={(-0.05,0.06)}, rotate=-45},
  %   y label style={at={(0.55,0.00)}, rotate=1},
  %   z label style={at={(-0.08,0.5)}},
  %   enlarge x limits=0,
  %   enlarge y limits=0,
  %   enlarge z limits=0,
  %   view={80}{10},
  %   ]

  %   % \addplot3 [scatter, only marks] table [y=y, x=x, z=z]{\tableMAP};
  %   \addplot3 [smooth, color=black, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJGT}; \label{ground_truth}
  %   \addplot3 [smooth, color=color_blue, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJV}; \label{uniform_sampling}
  %   \addplot3 [smooth, color=color_green, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJNS}; \label{normal_sampling}
  %   \addplot3 [smooth, color=color_orange, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJCOV}; \label{covariance_sampling}
  %   \addplot3 [smooth, color=color_red, line width=0.8pt] table [y=y, x=x, z=z]{\tableTRAJRISE}; \label{RISE_(proposed)}
            
  %   \coordinate (gt) at (axis description cs:1.45,0.75);
  %   \coordinate (legend) at (axis description cs:1.32,-0.12);

  % \end{axis}

  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-2mm, column sep=-1mm,
  %   nodes={rotate=0},
  %   font=\scriptsize,
  % ] at (gt) {
  %   \hspace{0mm} \ref{ground_truth} & ground truth  \\
  % };

  \node[fill=none] at (7.8, 3.0) {sampling:};
  % \node[fill=none,rotate=90] at (7.8, 2.3) {\textcolor{color_green}{\textbf{normal}}};
  % \node[fill=none,rotate=90] at (8.1, 2.3) {\textcolor{color_blue}{\textbf{uniform}}};
  % \node[fill=none,rotate=90] at (7.8, 1.0) {\textcolor{color_violet}{\textbf{covariance}}};
  % \node[fill=none,rotate=90] at (8.1, 1.0) {\textcolor{color_red}{\textbf{proposed}}};

  \node[fill=none,rotate=90] at (7.8, 1.7) {\textcolor{color_green}{\textbf{Rusinkiewicz et al.}}};
  \node[fill=none,rotate=90] at (8.1, 2.1) {\textcolor{color_blue}{\textbf{Voxelization}}};
  \node[fill=none,rotate=90] at (7.8, 0.06) {\textcolor{color_red}{\textbf{RMS}}};
  \node[fill=none,rotate=90] at (8.1, 0.5) {\textcolor{color_orange}{\textbf{Gelfand et al.}}};

  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-3mm, column sep=-1mm,
  %   nodes={rotate=0},
  %   font=\scriptsize,
  % ] at (legend) {
  %   % \hspace{0mm} sampling: \\
  %     \hspace{10mm} \rotatebox{90}{\hspace{3mm} \textcolor{color_violet}{\textbf{covariance}}}
  %   & \hspace{0mm} \rotatebox{90}{\hspace{4mm} \textcolor{color_red}{\textbf{proposed}}}\\
  %     \hspace{10mm} \rotatebox{90}{\hspace{0mm} \textcolor{color_green}{\textbf{normal}}}      
  %   & \hspace{0mm} \rotatebox{90}{\hspace{0mm} \textcolor{color_blue}{\textbf{uniform}}}\\
  % };

  % % ORIGINAL
  % \matrix [
  %   draw=none,
  %   matrix of nodes,
  %   anchor=south east,
  %   column 1/.style={anchor=base west},
  %   column 2/.style={anchor=base west},
  %   row sep=-3mm, column sep=-1mm,
  %   nodes={rotate=90},
  %   font=\scriptsize,
  % ] at (legend) {
  %                          % &                            & \hspace{-0mm} uniform\\
  %                          % &                            & \hspace{0mm} \ref{uniform_sampling} \\
  %                          % &                            & \hspace{-3mm} normal\\
  %                          % &                            & \hspace{-11mm} \ref{normal_sampling} \\
  %   % \hspace{-5mm} ground truth & \hspace{0mm} sampling: & \hspace{-2mm} proposed           \\
  %   % \ref{ground_truth}   & & \hspace{0mm}             \hspace{0mm} \ref{RISE_(proposed)}          \\
  %   % \hspace{0mm} \textbf{ground truth} & \\
  %   \hspace{0mm}           & \hspace{1.0mm} \textcolor{color_red}{\textbf{proposed}} \\
  %   \hspace{1mm} sampling: & \hspace{2mm} \textcolor{color_green}{\textbf{normal}} \\
  %   \hspace{0mm}           & \hspace{0mm} \textcolor{color_blue}{\textbf{uniform}} \\
  % };


\end{tikzpicture}
% \vspace{-0.2cm}


==> fig/residuals.tex <==
\tikzset{
  double -latex/.style args={#1 colored by #2 and #3}{
    -stealth,line width=#1,#2, % first arrow
    postaction={draw,-stealth,#3,line width=(#1)/3,
                shorten <=(#1)/3,shorten >=2*(#1)/3}, % second arrow
  }
}

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\begin{tikzpicture}[|every node/.style={
  draw=none,
  text=black},
  >=latex,
  font=\normalsize
  ]

  \node[anchor=south west,inner sep=0] (a) at (0,0) {
      \def\arraystretch{0}%
      \includegraphics[width=0.9\columnwidth]{\FIGPATH/residuals_bckg.png}%
    }; 
  \begin{scope}[x={(a.south east)},y={(a.north west)}]

    % %%{ useful grid to help you find coordinates for plotting the overlay
    % \draw[black, xstep=.1, ystep=.1] (0,0) grid (1,1);
    % \foreach \i in {0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1} {
    %   \node[align=center] at (\i, -0.05) {\i};
    %   \node[align=center] at (\i, 1.05) {\i};
    %   \node[align=center] at (-0.05, \i) {\i};
    %   \node[align=center] at (1.05, \i) {\i};
    % }
    % %%}

  % point to point
  \node[] at (0.23, 0.25)  {$\vect{p}$};
  \node[] at (0.12, 0.5) {$\vect{q}$};
  \node[text=color_red] at (0.12, 0.18) {$\vect{r}^{\bullet}$};

  % point to plane
  \node[] at (0.49, 0.1) {$\vect{p}$};
  \node[] at (0.463, 0.735) {$\vect{q}$};
  \node[] at (0.605, 0.29) {$\vect{n}$};
  \node[text=color_red] at (0.37, 0.115) {$\vect{r}^{\square}$};

  % point to line
  \node[] at (0.925, 0.12) {$\vect{p}$};
  \node[] at (0.77, 0.16) {$\vect{q}$};
  \node[] at (0.785, 0.495) {$\vect{v}$};
  \node[text=color_red] at (0.895, 0.38) {$\vect{r}^{|}$};

  \end{scope}

\end{tikzpicture}
\vspace{-0.2cm}

